Describing and Organizing Semantic Web and Machine Learning Systems in the SWeMLS-KG

In line with the general trend in artificial intelligence research to create intelligent systems that combine learning and symbolic components, a new sub-area has emerged that focuses on combining machine learning (ML) components with techniques developed by the Semantic Web (SW) community - Semantic Web Machine Learning (SWeML for short). Due to its rapid growth and impact on several communities in the last two decades, there is a need to better understand the space of these SWeML Systems, their characteristics, and trends. Yet, surveys that adopt principled and unbiased approaches are missing. To fill this gap, we performed a systematic study and analyzed nearly 500 papers published in the last decade in this area, where we focused on evaluating architectural, and application-specific features. Our analysis identified a rapidly growing interest in SWeML Systems, with a high impact on several application domains and tasks. Catalysts for this rapid growth are the increased application of deep learning and knowledge graph technologies. By leveraging the in-depth understanding of this area acquired through this study, a further key contribution of this paper is a classification system for SWeML Systems which we publish as ontology.

==> tables/conceptsDescription.tex <==
\begin{table}[htb]
\caption[Short descriptions of the main classes of the SWeMLS ontology]{Short descriptions of the main classes of the SWeMLS ontology}
\label{tab:conceptsDescription}
\centering
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{1.2}
    \begin{tabularx}{\textwidth}{ l X }
    
    \hline
        \textbf{Class} & \textbf{Description} \\
     
    \hline
        System & Systems that rely on both Semantic Web resources and Machine Learning components (SWeMLS). \\
        Pattern & A standardized representation of the processing flows and the roles of the SW and ML components in a SWeML system.\\
        Processor & A notion to represent the algorithmic module. It uses one or more Instances as input, applies one or more Models, and outputs one or more Instances. \\
        % A Processor may use other procedures, such as data pre-processing.\\
            % \hline
            
    \hline
        Task & The task that a SWeML system seeks to address.\\
        Domain & The application domain of a SWeML system. \\
        Area & The application area of a SWeML system. \\
    
    \hline
        Model & A set of assumptions, data, and inferences used to represent an entity or state mathematically.\\
        \hspace{7pt} StatisticalModel & A mathematical relationship between one or more random variables and other non-random variables. \\   
        \hspace{7pt} SymbolicModel & It shows the connections between different "concepts" (entities). The meaning that underlies information is formally represented by semantic technologies.\\
        
    \hline
        Instance & An example or single occurrence of something.\\
        \hspace{7pt} Data & Facts and statistics collected together and used as a basis for reasoning, discussion or calculation.\\
        \hspace{7pt} Symbol & A representation of symbolic data such as semantic entities or relations.\\
    
    \hline
        System Maturity & The classification of a SWeML system's maturity level.\\
        Documentation & Documentation properties about infrastructure, provenance, evaluation and other properties of a SWeML system. \\
        Paper & Papers in which such SWeML systems are reported. It contains information about author's country, keywords, title and other information of a paper.\\
        
    \hline
    
    
    \end{tabularx}
\end{table}

==> tables/swemlsOntologyDetails.tex <==

\begin{table}[htb]
\caption{SWeMLS Knowledge Graph statistics}
\label{table:swemls-statistics}

\footnotesize
\centering
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l r}

\hline

Metrics & Count \\
\hline
Classes &
	47 
    \\


Data properties &
	17  
    \\

Object properties &
	55  
    \\

Individuals &
	4510  
    \\

Axioms &
	30587
    \\

    \hline

\end{tabular}


\end{table}



